ReCLIP: Refine Contrastive Language Image Pre-Training with Source Free Domain Adaptation

Large-scale Pre-Training Vision-Language Model such as CLIP has demonstrated outstanding performance in zero-shot classification, e.g. achieving 76.3% top-1 accuracy on ImageNet without seeing any example, which leads to potential benefits to many tasks that have no labeled data. However, while applying CLIP to a downstream target domain, the presence of visual and text domain gaps and cross-modality misalignment can greatly impact the model performance. To address such challenges, we propose ReCLIP, the first source-free domain adaptation method for vision-language models, which does not require any source data or target labeled data. ReCLIP first learns a projection space to mitigate the misaligned visual-text embeddings and learns pseudo labels, and then deploys cross-modality self-training with the pseudo labels, to update visual and text encoders, refine labels and reduce domain gaps and misalignments iteratively. With extensive experiments, we demonstrate ReCLIP reduces the average error rate of CLIP from 30.17% to 25.06% on 22 image classification benchmarks. Code available at https://github.com/michiganleon/ReCLIP_WACV.

==> sections/introduction_backup.tex <==
% It has been more than a decade since we benefit from the breakthrough of deep learning. 
%Deep learning, in the paradigm of fully supervised learning, has been benefiting the Artificial Intelligence research for more than a decade. However, crucial limitation presents in such paradigm, such as interpretability and transfer-ability. Deep learning models trained on one task is often highly biased towards that particular task and can not be trivially extended or adapted to a new task. 

%Meanwhile, human brain 

% Image classification, the most simple but also most fundamental problem in the field of computer vision, has been formulated as a task that given an input query images, to predict a label within a list of pre-defined categories. Since more than a decade ago, with the help from large-scale human-labeled dataset such as ImageNet\xuefeng{ref} and progress in deep learning, the prediction accuracy of fully supervisory trained models have already outperformed human benchmarks\xuefeng{ref}. The progress was exciting, but there is still a long way toward a human-level ``general purpose" computer vision system, especially on perspectives such as robustness\xuefeng{ref}, interpretability\xuefeng{ref} and ability to fast adapt to new concepts\xuefeng{ref}. 

% The classic paradigm of image classification, as shown in the top row of Figure \ref{fig:intro}, typically requires a list of fixed pre-defined categories, thousands of human-labeled data per category, and fully supervised training. To alleviate this heavy label and training burden on downstream tasks, and also to improve deep learning models' ability to adapt, various Domain Adaptation settings and techniques have been studied and developed. Depends on the whether or not there are novel concepts (with respective to the training domain) in the testing domain, there are closed-set Domain Adaptation\xuefeng{ref} and open-set Domain Adaptation tasks\xuefeng{ref}. Depends on the amount of exemplary data available on the testing domain, there are fully-supervised\xuefeng{ref}/semi-supervised\xuefeng{ref}/few-shot\xuefeng{ref} and unsupervised Domain Adaptation\xuefeng{ref} tasks. Among those settings, the most challenging yet most practical one is open-set unsupervised domain adaptation tasks, which is also known as the zero-shot learning task\xuefeng{ref}. 

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{figures/intro.pdf}
%     \caption{A demonstration of different learning paradigms in Image Classification task. Compare to the classic supervised and transfer learning, our method can be applied on any novel classification tasks without requiring any additional supervision; compare to zero-shot learning models (CLIP\cite{radford2021learning}), our method obtains significant performance improvement, with only additional requirement of a fast tuning process. \xuefeng{the figure can be improved, maybe larger font?}}
%     \label{fig:intro}
% \end{figure}

% The most intuitive distinction between a fully-supervisory trained deep learning model and human intelligence system is that human typically does not treat vision as an independent problem, which requires thousands of examples to learn from scratch. With a mature cognitive system, human typically can learn new concepts as an extension to the related ideas that is already in the system. Recently, CLIP (Contrastive Language-Image Pre-training)\cite{radford2021learning}, a large-scale "foundation" model from OpenAI, has proposed an alternative paradigm as shown in the third row of Figure \ref{fig:intro}, which learns to match image towards their text descriptions, rather than just towards simplified category abstraction (labels) with no semantic meaning. The new paradigm slightly loosen the strictness requirement in data-collection process. With the help of Wikipedia and Google image search, people collected a dataset with 400M image-text pairs, over 500K concepts. (For comparison, ImageNet has 14M images over 22k categories, which took 3 years to collect and label). With the help of unified language-vision space and the large-scale training data, CLIP becomes very robust and is able to be applied on new images and concepts without any further training, which they referred as the capability of zero-shot image classification. CLIP's astonishing performance in many domain and its capability of performing zero-shot classification have lead to an exciting future. Without requirement of extra supervision or training time, CLIP can be directly deployed onto many applications. 
% \xuefeng{Shrink the above contents to shorter version, focus more on our task and solution}

% However, CLIP is still far from perfect. In fact, we can still observe few conditions which can cause reduced CLIP performance, such as inaccurate text description of fine-grained categories or visual domain gap caused by different resolution or image manipulation. These conditions suggest that CLIP can be improved.

% The core idea of CLIP is to build an unified visual-text embedding space to perform classification. However, our further analysis suggests that CLIP's embeddings spaces might not be well aligned as expected in many cases, possibly due to the text or visual domain gap on test domain. 

% Therefore, it is necessary to be able to perform source-free unsupervised domain adaptation to refine CLIP’s classification accuracy performance on target dataset, by closing the gap between visual & language representation spaces.

% To the best of our knowledge, we are the first work that adapts large-scale vision-language model without requiring any label on target domain. 

% In this project, our main contribution can be summarized as four-folds:
% \begin{itemize}
%     \item As the first work that studies the unsupervised adaptation problem of "foundation" vision-language model, we enhanced the CLIP's generalization ability to be applied onto novel test domain without requiring any label;
%     \item We identified and addressed a mis-alignment issue between CLIP's visual and language embeddings spaces, with a novel proposed feature projection technique; 
%     \item We designed a novel co-learning algorithm by creating two distinctive model instances that compliment each other, which stabilized the noisy unsupervised training;
%     \item With extensive experiments over different learnable modules and optimization strategies, we come up with a model configuration that produces consistent and significant improvements over the vanilla CLIP model, and also outperforms all the baseline methods;
% \end{itemize}


%\xuefeng{re-doing the intro: 1. Shift of paradigm, CLIP+Zero-Shot is the future; 2. CLIP is not yet perfect; 3. Current UDA can not solve CLIP's problem; 4. What did we do.}

% Image classification, the most simple yet most fundamental problem in the field of computer vision, has been formulated as a task that given an input query images, to predict a label within a list of pre-defined categories. Since more than a decade ago, with the help from large-scale human-labeled dataset such as ImageNet\xuefeng{ref} and progress in deep learning, the prediction accuracy of fully supervisory trained models have already outperformed human benchmarks\xuefeng{ref}. The progress was exciting, but there is still a long way toward a human-level ``general purpose" computer vision system, especially on perspectives such as robustness\xuefeng{ref}, interpretability\xuefeng{ref} and ability to fast adapt to new concepts\xuefeng{ref}. 

% The classic paradigm of image classification, as shown in the top row of Figure \ref{fig:intro}, typically requires a list of fixed pre-defined categories, thousands of human-labeled data per category, and fully supervised training. To alleviate this heavy label and training burden on downstream tasks, and also to improve deep learning models' ability to adapt, various Domain Adaptation settings and techniques have been studied and developed. Depends on the whether or not there are novel concepts (with respective to the training domain) in the testing domain, there are closed-set Domain Adaptation\xuefeng{ref} and open-set Domain Adaptation tasks\xuefeng{ref}. Depends on the amount of exemplary data available on the testing domain, there are fully-supervised\xuefeng{ref}/semi-supervised\xuefeng{ref}/few-shot\xuefeng{ref} and unsupervised Domain Adaptation\xuefeng{ref} tasks. Among those settings, the most challenging yet most practical one is open-set unsupervised domain adaptation tasks, which is also known as the zero-shot learning task\xuefeng{ref}. 


==> sections/results_backup.tex <==
\begin{table*}[ht]
\small
\resizebox{\textwidth}{!}{
\setlength{\tabcolsep}{0.2em} % for the horizontal padding
{\renewcommand{\arraystretch}{1.2}% for the vertical padding
\begin{tabular}{ccccccccccccccccccccccccc}
              &      \rotatebox{90}{Avg Acc} &   \rotatebox{90}{AID\cite{xia2017aid}} & \rotatebox{90}{Birdsnap\cite{berg2014birdsnap}} & \rotatebox{90}{Caltech101\cite{caltech101}} & \rotatebox{90}{CIFAR10\cite{cifar}} & \rotatebox{90}{CIFAR100\cite{cifar}} & \rotatebox{90}{Country211\cite{radford2021learning}} & \rotatebox{90}{DTD\cite{dtd}} & \rotatebox{90}{EuroSAT\cite{helber2019eurosat}} & \rotatebox{90}{FER2013\cite{fer}} & \rotatebox{90}{FGVC\cite{fgvc}} & \rotatebox{90}{Flowers\cite{flower102}} & \rotatebox{90}{Food101\cite{bossard2014food}} & \rotatebox{90}{GTSRB\cite{GTSRB}} & \rotatebox{90}{ImageNet\cite{deng2009imagenet}} & \rotatebox{90}{MNIST\cite{deng2012mnist}} & \rotatebox{90}{Oxford Pet\cite{pet}} & \rotatebox{90}{PCam\cite{pcam}} & \rotatebox{90}{SST2\cite{radford2021learning}} & \rotatebox{90}{RESISC45\cite{resisc45}} & \rotatebox{90}{Cars\cite{cars}} & \rotatebox{90}{STL10\cite{stl}} & \rotatebox{90}{SUN397\cite{xiao2010sun}}  \\ \hline
%Image Number     &       & 1.5K          & 2,149          & 9,146          & 10K         & 10K         & 21.1K         & 1,880          & 5K          & 3,574          & 3,333          & 6,149          & 25.25K         & 12.63K         & 50K         & 10K         & 3,669          & 32,768         & 1,821          & 25.2K         & 8,041          & 8K          & 19.85K         \\
%Class Number     &       & 30             & 500            & 102            & 10             & 100            & 211            & 47             & 10             & 8              & 100            & 102            & 102            & 43             & 1,000          & 10             & 37             & 2              & 2              & 45             & 196            & 10             & 397            \\ \hline
CLIP \textit{report}   &     70.08   & -              & 48.30          & 92.6*          & 96.20          & 77.90          & \textbf{32.70} & 55.30          & 59.90          & 57.50          & 36.1*          & 78.7*          & 92.90          & 50.30          & 75.30          & 87.20          & 93.50          & 58.80          & 64.00          & 71.60          & 77.3*          & 99.30          & 67.70          \\
CLIP \textit{single} & 65.53 & 61.30 & 51.88 & 92.02 & 95.19 & 77.18 & 25.78 & 52.50 & 56.03 & 52.22 & 30.18 & 74.19 & 92.56 & 45.57 & 73.46 & 52.63 & 93.21 & 57.75 & 52.39 & 63.29 & 76.45 & 99.47 & 66.42  \\
CLIP \textit{multi} &     69.83   & 68.73          & 52.48          & 91.63          & 95.60          & 78.22          & 31.84          & 55.37          & 60.00          & 56.39          & 31.59          & 79.04          & 93.08          & 50.59          & 75.52          & 76.23          & 93.62          & 62.43          & 68.92          & 69.66          & 77.88          & 99.36          & 67.97          \\ \hline

%SHOT Pseudo Label \kz{move to suppl} &     59.38   & 78.10          & 0.27           & 90.72          & 95.91          & 74.39          & 21.88          & 56.54          & 80.58          & 35.86          & 1.45           & 1.45           & 91.54          & 46.60          & 0.10           & 76.66          & 92.40          & 64.97          & 70.29          & 79.11          & 77.23          & 99.22          & 71.03          \\ 
%Label Propagation \kz{move to suppl} &     72.54   & 74.50          & 43.25          & 91.91          & 96.56          & 81.40          & 26.30          & 59.04          & 73.36          & 57.15          & 36.33          & 82.55          & 93.95          & 60.64          & 25.11          & 82.85          & 94.77          & 62.46          & 68.86          & 77.63          & 77.66          & 99.52          & 70.54          \\ \hline
%SHOT              &     36.48   & 42.93                & 0.27                 & 5.05                 & 95.84                & 79.47                & 0.55                 & 55.32                & 24.03                & 18.03                & 1.65                 & 1.43                 & 1.00                 & 32.84                & 0.10                 & 84.14                & 93.51                & 67.61                & 49.92                & 2.05                 & 0.6                  & 99.28                & 46.9                 \\
%SHOT \textit{peak} &     55.49             & 70.03                & 51.67                & 91.85                & 96.31                & 79.47                & 0.67                 & 55.48                & 24.03                & 54.42                & 31.98                & 8.39                 & 1.89                 & 53.21                & 0.10                 & 87.99                & 93.62                & 67.61                & 70.29                & 54.76                & 77.35                & 99.40                & 50.29               \\ \hline
AaD    & 46.53 & 69.83 & 52.42 & 91.45 & 96.54 & 80.18 & 0.47  & 55.43 & 11.12 & 16.91 & 32.37 & 78.61 & 0.99  & 51.26 & 0.11  & 89.81 & 93.62 & 49.95 & 49.92 & 2.51  & 0.52  & 99.41 & 0.25\\
AaD \textit{peak} & 71.79  & 70.33 & 52.58 & 91.93 & 96.55 & 80.46 & 31.90 & 55.59 & 76.18 & 55.67 & 32.43 & 79.22 & 93.04 & 52.83 & 75.53 & 91.95 & 93.73 & 64.03 & 68.97 & 71.01 & 77.96 & 99.42 & 67.96 \\ \hline
% POUF-full & 67.60 & 66.23 & 52.53 & 92.90 & 96.38 & 75.86 & 28.25 & 58.46 & 73.99 & 55.50 & 33.90 & 74.89 & 92.76 & 53.58 &  & 57.11 & 93.80 & 53.25 & 48.49 & 66.50 & 76.96 & 99.44          & 68.83 \\
% POUF-full \textit{peak} & 70.46 & 66.23 & 53.12 & 93.19 & 96.40 & 80.80 & 28.25 & 58.51 & 73.99 & 56.20 & 34.00 & 76.79 & 92.80 & 53.58 &  & 93.60 & 94.60 & 66.80 & 48.76 & 66.84 & 76.97 & 99.50 & 68.83 \\
% POUF-prompt     & 66.07 & 75.43 & 40.42 & 87.73 & 96.94 & 76.40 & 15.61 & 49.84 & 61.46 &       & 31.95 & 77.10 & 91.30 & 56.19 &  & 72.50 & 94.41 & 46.60 & 44.98 & 72.81 & 70.66 & 99.58          & 59.50 \\
% POUF-prompt \textit{peak}     & 70.72 & 76.77 & 49.25 & 89.98 & 96.94 & 77.93 & 26.10 & 57.12 & 69.57 &       & 32.97 & 79.25 & 92.27 & 57.09 &  & 76.32 & 94.99 & 66.79 & 52.06 & 75.83 & 75.15 & \textbf{99.65} & 68.37 \\ \hline
POUF-full                       & 69.73 & 64.83 & 52.91 & 92.97 & 96.06 & 80.39 & 28.19 & 56.65 & 67.95 & 55.92 & 32.88 & 75.62 & 92.71 & 51.47 & 73.05 & 91.22 & 94.20 & 66.57 & 48.22 & 67.54 & 76.72 & 99.50          & 68.38 \\
POUF-full \textit{peak}         & 69.76 & 64.87 & 52.96 & 92.97 & 96.06 & 80.39 & 28.22 & 56.75 & 67.95 & 55.92 & 32.91 & 75.62 & 92.73 & 51.47 & 73.06 & 91.22 & 94.20 & 66.75 & 48.60 & 67.54 & 76.72 & 99.53 & 68.38 \\ \hline
% POUF-prompt                     & 65.48 & 76.50 & 40.74 & 87.46 & 96.57 & 76.98 & 16.14 & 51.17 & 60.92 & 33.21 & 32.37 & 77.82 & 91.12 & 55.55 & 68.05 & 73.11 & 94.39 & 61.67 & 44.07 & 73.90 & 69.64 & 99.58          & 59.60 \\
% POUF-prompt \textit{peak}       & 69.91 & 76.50 & 49.25 & 89.99 & 96.76 & 77.93 & 26.10 & 57.13 & 69.57 & 51.96 & 32.37 & 79.25 & 92.27 & 57.09 & 73.91 & 76.32 & 94.60 & 66.79 & 52.09 & 75.09 & 75.15 & \textbf{99.59} & 68.37 \\ \hline
% Label Propagation &     72.54   & 74.50          & 43.25          & 91.91          & 96.56          & 81.40          & 26.30          & 59.04          & 73.36          & 57.15          & 36.33          & 82.55          & 93.95          & 60.64          & 25.11          & 82.85          & 94.77          & 62.46          & 68.86          & 77.63          & 77.66          & 99.52          & 70.54          \\ 
ReCLIP            &     74.94 & 77.97          & 52.96          & 93.02          & 96.95          & 82.32          & 31.92          & 60.85          & 78.75          & 58.07          & 36.63          & 82.05          & 94.15          & 66.81          & 75.81          & 90.88          
& 95.61          & 70.15          & 73.48          & 78.41          & 77.96          & 99.58          & 74.41          \\ 
ReCLIP \textit{peak} &   \textbf{75.85}    & \textbf{79.27} & \textbf{53.28} & \textbf{93.10} & \textbf{97.04} & \textbf{83.42} & 31.95          & \textbf{61.38} & \textbf{79.94} & \textbf{58.29} & \textbf{38.70} & \textbf{83.14} & \textbf{94.18} & \textbf{69.14} & \textbf{76.01} & \textbf{97.11} & \textbf{96.05} & \textbf{70.56} & \textbf{73.48} & \textbf{79.31} & \textbf{79.26} & \textbf{99.59} & \textbf{74.53} \\ \hline
\end{tabular} 
}
}
\caption{Classification accuracies (\%) on 22 benchmarks. * on FGVC, Caltech101, Oxford-IIIT Pet and Flowers102, CLIP reported mean-class-accuracy. All other scores in this table are top-1 accuracy.}
\label{tab:main}
\end{table*}

\begin{table}[]
\resizebox{\linewidth}{!}{
\begin{tabular}{cccccc}
              & Avg       & Ar            & Cl        & Pr        & Rw     \\ \hline
CLIP \textit{single}                     & 82.45          & 82.70          & 68.10          & 89.10          & 89.90          \\ \hline
POUF-prompt              & 84.28          & 83.70          & 71.20          & 91.40          & 90.80          \\
POUF-full                & 86.10          & \textbf{86.20} & 73.80          & 92.70          & 91.70          \\ \hline
Label Propagation & 84.94          & 83.27          & 73.49          & 91.89          & 91.09          \\
ReCLIP  & \textbf{86.99} & 86.11          & \textbf{75.97} & \textbf{93.90} & \textbf{92.01} \\ \hline
\end{tabular}
}
\label{office}
\caption{Comparison of official POUF scores \cite{tanwisuth2023pouf} with ReCLIP on Office-Home\cite{venkateswara2017deep}, both with single-prompt CLIP as base model.}
\end{table}

\begin{table}[t]
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ccccc}
    \multicolumn{1}{l}{}            & CIFAR10        & CIFAR100       & AID             & SUN397    \\ \hline
    Vanilla CLIP                    & 95.54          & 76.48          & 64.87           & 67.25     \\
    Label Propagation               & 96.38          & 80.66          & 74.73           & 70.54     \\
    ReCLIP-V                        & 96.69          & 80.84          & 79.47           & 67.15     \\
    ReCLIP-T                        & 96.50          & 81.10          & 79.07           & 70.12     \\
    ReCLIP (w/o Label Sharing)      & 97.40          & 82.80          & 80.01           & 71.10     \\
    ReCLIP (w/ Label Sharing)       & \textbf{97.48} & \textbf{84.14} & \textbf{82.53}  & \textbf{71.34} \\ \hline  
    \end{tabular}
    }
    \caption{Comparison of classification accuracy with different version ReCLIP on ablation datasets. ReCLIP with Label Sharing (Figure \ref{fig:model3}) is shown to be most effective compared to ReCLIP-V, ReCLIP-T (Figure \ref{fig:model1}) and their simply assembled predictions (ReCLIP w/o Label Sharing).}
    \label{abla:method}
\end{table}


\subsection{Zero-Shot Classification Benchmarks}
\label{sec:main}
In Table \ref{tab:main} we present the source-free adaptation accuracy of ReCLIP and baseline methods over 22 datasets. Besides the accuracy from final epoch of self-training, we report the accuracy from the peak-performing epoch for AaD, POUF and ReCLIP as well, denoted as \textit{peak}.

As shown in Table \ref{tab:main}, ReCLIP achieves consistent and significant improvements over CLIP on 21 datasets and comparable performance on Country 211. ReCLIP improves the averaged top-1 accuracy of CLIP by 5.11\% at the final epoch, and by 6.02\% over the 22 datasets without accessing any labeled data, which also outperforms both baseline adaptation methods AaD, POUF with clear margin. 

% In comparison with CLIP, ReCLIP decreases CLIP's average error rates from 30.17\% to 25.06\%, with a 17\% relative improvement. ReCLIP achieves further gains at peak performance, lowering average error rates to 124.15\% with 20\% relative improvement over CLIP. 

Comparing to AaD, although AaD achieves 1.96\% improvements over CLIP at its peak epochs, it encounters drastic performance drop at final epochs that lose 25.26\% of the averaged accuracy, due to collapsed unsupervised training on target datasets such as Food101, SUN397, ImageNet, etc. Meanwhile, ReCLIP maintains the performance at final epochs, and only has 0.91\% differences from peak epochs to final epochs. These results suggest that the high-quality commonly-agreed pseudo labels produced by ReCLIP have stabilized the noisy self-training and have prevented the model from collapsing.

\modification{
POUF-prompt and POUF-full achieve reasonable improvements over single-prompt CLIP on many of the datasets, but fail to improve on certain datasets such as Birdsnap, FER2013, Food101, etc. 
Due to  memory (POUF-full) and  design restrictions (POUF-prompt), POUF can only generate the class names embeddings with the default template \texttt{``A photo of \{classname\}'' }, while both ReCLIP and CLIP use the averaged class name embeddings with a list of various templates that are designed fit various target domains. Such difference in the prompt templates limits the initial performance of POUF, and sometimes cancels out the adaptation improvements brought by POUF with an result performance weaker than multi-prompt CLIP. In between POUF-prompt and POUF-full, we observe that POUF-prompt experience less such impact from the template restriction (e.g. AID, Flowers102, GTSRB and RESISC45.), which indicates the effectiveness of its learnable prompt.
}

% To compare with SHOT, we observe SHOT achieves decent performance 
% On simple datasets such as MNIST, STL10, CIFAR10, and CIFAR100 where SHOT was originally tested on\cite{liang2020we}, SHOT did not drop much performance on the final epoch compared to its peak. However, on many other datasets, we observe a significant performance drop at the final epochs. Comparing the peak and final epoch performance, SHOT lost 19.01\% while ReCLIP only lost 0.91\%. This indicates that our self-training algorithm is effective in stabilizing the noisy unsupervised adaptation process. On the other hand, even at peak epochs, SHOT gets significantly less improvement than ReCLIP. One possible reason is that SHOT only updates the visual feature extractor and keeps the classifier part frozen, which has limited its performance. As we mentioned in Section \ref{limitation_clip}, the classification weights from CLIP can also be improved, especially when the category names are not accurate. This comparison indicates the advantage of ReCLIP in adapting vision-language models.

% As both SHOT and ReCLIP use pseudo labels to perform adaptation, we have also observed that the pseudo labels from ReCLIP are more stable than the ones by SHOT. Detailed comparison on pseudo label quality of SHOT and ReCLIP is provided in the supplementary materials. 

% To compare first epoch pseudo label accuracy generated by SHOT and by our version Label Propagation, we observe that SHOT's clustering algorithm achieves decent performance on many datasets, but fails on Birdsnap, FER2013, FGVC, Flowers102, ImageNet with no clear pattern on the condition causing its collapsed performance. The unstable performance of pseudo label generation has also influenced the performance of SHOT. Label Propagation obtains more consistent improvement on pseudo label accuracy, only except on Birdsnap and ImageNet which have more than 500 categories, as we discussed in Section \ref{details}. More discussion on pseudo label generation is covered in Section \ref{abla:cluster}. 

For Country211, as we briefly mentioned in Section \ref{limitation_clip}, it is designed to predict geo-location based on visual appearance, while CLIP might tend to describe the image from actual content and texture. As shown in \cite{radford2021learning}, CLIP can only achieve 42.9\% after its classifier is fine-tuned in the fully supervised way. Therefore, it is challenging to obtain improvement during unsupervised adaptation. 
% \xh{TODO: address table 3}

% \begin{table}[]
% \resizebox{\linewidth}{!}{
% \begin{tabular}{cccc}
% Methods     & Update Parameter                  & BS $\times$ Iter              & Time (S)           \\ \hline
% AaD         & Visual Encoder \& Classifer       & 64 $\times$ 5000              & 5560    \\
% POUF-full   & Full                              & 32 $\times$ 10000             & 32482   \\
% POUF-prompt & Text Prompt                       & 32 $\times$ 10000             & 25860    \\
% ReCLIP      & Layer-Norm                        & 64 $\times$ 5000              & 16656    \\ \hline
% \end{tabular}
% }
% \caption{Runtime comparison on SUN397 with single V100 GPU. \xh{will update}}
% \label{runtime}
% \end{table}

\noindent\textbf{Runtime and Inductive Performance} %Despite the original CLIP pre-training took 73728 GPU-hours on V100 GPU~\cite{radford2021learning}),
Self-training of ReCLIP is very efficient, which completes adaptation in only 0.5 to 5 GPU-Hour on V100, depending on the target dataset size. Note that this adaptation time is a one-time effort on each target domain and ReCLIP can then inference on unseen data from the same domain without re-training.
Besides the transducitve results provided in Table \ref{tab:main}, we also run ReCLIP in a inductive setting, where ReCLIP performs self-training on the training split of a dataset (0.5 to 5 GPU-Hour), and inference on the test split (similar to CLIP inference time). ReCLIP achieves similar improvements in the inductive setting: 96.92\%, 82.30\% and 79.87\% accuracy on the test sets of CIFAR10, CIFAR100 and AID, respectively.
%The inductive results indicate ReCLIP is capable of maintaining its performance on new and unseen examples from the same domain.
More results in inductive setting is also available in Section \ref{sec:abla}.

    \begin{table}[t]
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lcccc}
                                & AID   & CIFAR10   & CIFAR100 & SUN397  \\ \hline
    Vanilla CLIP                & 68.80                     & 95.59                         & 78.21              & 67.97           \\ \hline
    Hierarchical Clustering     & 55.20                     & 36.52                         & 9.27               & 46.93           \\
    Spectrum Clustering         & 68.10                     & 61.25                         & 57.35              & 27.45           \\
    $k$-means Clustering        & 72.73                     & 95.07                         & 49.43              & 43.66           \\ \hline
    $k$-NN Classifier ($P_0$)     & 72.30                     & 93.74                         & 69.46            & 60.72             \\
    $k$-NN Classifier ($P_1$)     & 72.76                     & 95.77                         & 77.81            & 63.07             \\
    $k$-NN Classifier ($P_2$)     & 72.43                     & 95.76                         & 78.19            & 63.29             \\ \hline
    Label Propagation ($P_0$)   & 60.80                     & 94.01                         & 63.58              & 51.77           \\ 
    Label Propagation ($P_1$)   & 60.43                     & 96.23                         & 45.41              & 33.41          \\ 
    Label Propagation ($P_2$)   & \textbf{76.36}            & \textbf{96.31}                & \textbf{81.56}     & \textbf{70.44}           \\ \hline
    \end{tabular}
    }
    \caption{Pseudo label accuracy with different methods. Label Propagation on projection space $P_2$ is shown to be the most effective and stable method in generating accurate pseudo labels. }
    \label{table:clustering}
    \end{table} 



\subsection{Domain Adaptation Benchmark}



\subsection{Ablations Studies}
\label{sec:abla}
    In this section, we present the ablation studies on choices of learnable modules, pseudo label generation, and a comparison of different ReCLIP versions.
    We use AID, CIFAR10, CIFAR100 and SUN397 as our ablation datasets, and the test set of each dataset is equally split  into two fixed partitions. We report all ablation results in an inductive manner where models are first trained on partition 1 and then evaluated on partition 2. Note that results in this section is not directly comparable to \ref{sec:main} because the different evaluation partition.
    
    % In Table 4.1 we provided the baseline performances of CLIP in zero-shot and linear-evaluation settings. 

    %\subsubsection{Baseline and Experiment Setup}
    % \begin{table*}[]
    % \resizebox{\textwidth}{!}{
    % \begin{tabular}{ccccccc}
    % Test Partition             & Training Partition    & Loss                         & CIFAR10 & CIFAR100 & AID   & Note                                                      \\ \hline
    % Full Validation (Reported) & None                  & Zero-Shot                    & 95.70   & 77.50    & -     & reported baseline performance                             \\
    % Full Validation (Reported) & Training Set          & Fully Supervised Linear Eval & 97.90   & 87.40    & -     & reported optimal performance with   fixed visual features \\ \hline
    % 50\% Validation (Our)      & None                  & Zero-Shot                    & 95.30   & 69.60    & 60.10 & tested baseline performance, single prompt                \\
    % 50\% Validation (Our)      & None                  & Zero-Shot                    & 95.54   & 76.48    & 64.87 & tested baseline performance, 80 prompt                    \\
    % 50\% Validation (Our)      & Other 50\% Validation & Fully Supervised Linear Eval & 97.78   & 84.30    & 95.60 & tested optimal performance with   fixed visual features  
    % \end{tabular}
    % }
    % \caption{}
    % \label{tab:abla}
    % \end{table*}
    \begin{table}[ht]
    \setlength{\tabcolsep}{0.2em}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ccccc}
                      & CIFAR10                                     & CIFAR100                                      & AID                                   & SUN397     \\
                      & Init  $\rightarrow$   Adapt            & Init $\rightarrow$ Adapt                 & Init $\rightarrow$ Adapt         & Init         $\rightarrow$ Adapt           \\ \hline
    SLIP (ViT-L/16)   & 89.45     $\rightarrow$   \textbf{91.80}    & 56.69  $\rightarrow$ \textbf{67.61}           & 48.13   $\rightarrow$\textbf{64.07}   & 55.56   $\rightarrow$ \textbf{65.28} \\
    DeCLIP (ViT-B/32) & 90.57     $\rightarrow$   \textbf{94.50}    & 66.58  $\rightarrow$ \textbf{77.10}           & 53.53  $\rightarrow$\textbf{65.93}    & 63.05   $\rightarrow$ \textbf{66.90} \\ \hline
    CLIP (RN50)       & 71.46     $\rightarrow$   \textbf{82.73}    & 42.32  $\rightarrow$ \textbf{53.15}           & 53.43  $\rightarrow$\textbf{65.97}    & 59.76   $\rightarrow$ \textbf{65.38}      \\
        CLIP (ViT-B/32)   & 89.83     $\rightarrow$   \textbf{92.15}    & 65.25  $\rightarrow$ \textbf{71.09}       & 60.83  $\rightarrow$\textbf{76.80}    & 62.96   $\rightarrow$ \textbf{68.30} \\ \hline
    \end{tabular}
    }
    \caption{Ablation Studies on the effectiveness of ReCLIP on different model architecture and pre-training strategies.}
    \label{effectiveness}
    \end{table}
    
    \subsubsection{Effectiveness of ReCLIP Components}
    In Table \ref{abla:method} we present the comparison between different versions of ReCLIP. As shown, Label Propagation can create pseudo labels with significantly improved accuracy compared to vanilla CLIP. On the top of Label Propagation, both ReCLIP-V and ReCLIP-T (Figure~\ref{fig:model1}) are shown to be effective in providing further improvements. 
    In ReCLIP(w/o Label Sharing) we present the result by simply assembling predictions from separately trained ReCLIP-V and ReCLIP-T at inference time. Comparing the last two rows of Table \ref{abla:method} we observe that ReCLIP~(w/ Label Sharing) has clear improvement over ReCLIP~(w/o Label Sharing), which indicates that the commonly agreed pseudo-labels stabilizes the noisy adaptation process and improved both ReCLIP-V and ReCLIP-T to achieve better performance. 
        



    \subsubsection{Comparison on Pseudo Label Generations}\label{abla:cluster}
    
    In Table \ref{table:clustering}, we compare methods in pseudo label generation.
    For clustering based methods, we assign the same pseudo labels for examples from the same cluster, based on the in-cluster majority vote; 
    For $k$-NN Classifier and Label Propagation methods, we experiment them on original CLIP feature space $P_0$, and on projection spaces $P_1, P_2$ as described in Figure \ref{fig:project}.
    For $k$-NN Classifiers, we assign each example with the major vote prediction within its $k$-nearest-neighborhood, with $k$ equal to the average sample count per class.  
    For Label Propagation on $P_0$, we select the example with the highest confidence from each class as the labeled example to perform label propagation as a baseline. 
    Label Propagation on $P_1, P_2$ are as described in Section \ref{sec:ps}.
    
    Table \ref{table:clustering} indicates $k$-NN based methods achieve better performance on projection spaces $P_1$ are $P_2$, which indicates the effectiveness of $P_1, P_2$ in refining CLIP's visual embeddings. On Label Propagation methods, $P_2$ gives a significant improvement over $P_0, P_1$, indicating its effectiveness in aligning CLIP's visual and text embeddings. 


    \subsubsection{Comparison on other Vision-Language Models}

    ReCLIP is designed to improve the classification performance of visual-language models in general, not only on CLIP. We tested the effectiveness of ReCLIP on SLIP\cite{mu2022slip} and DeCLIP\cite{li2021supervision}, both of these improved CLIP by adding self-supervision learning objectives during pre-training. We have also tested ReCLIP on other versions of CLIP with smaller architectures. As shown in Table \ref{effectiveness}, ReCLIP demonstrates steady and significant improvements on various vision-language models and architectures.



    % \subsection{Efficiency and Robustness}
    % It took 73728 GPU-hours (V100 GPU) train the original CLIP model~\cite{radford2021learning}, while the ReCLIP takes only 0.5 to 5 GPU-Hour for adaptation on the same GPU, depends on the unlabeled training size. Note that the adaptation training is an one-time cost for user on their test domain as ReCLIP maintains its performance on unseen data from the same test domain after adaptation. In Table \ref{generalization} we demonstrate the effectiveness of ReCLIP across different test data within the same test domains (low-resolution objects from CIFAR10/100, satellite images from AID and RESISC45).

    % \subsubsection{Effectiveness of ReCLIP on Unseen Examples}

    % In Table \ref{tab:main} we demonstrate ReCLIP performance in the transductive setting, where ReCLIP is adapted and tested on the same examples. In this section, we evaluate ReCLIP in the inductive setting, where ReCLIP has never seen the test examples during its adaptation process. We sampled 10,000/10,000/1,500 examples from the official dataset training set of CIFAR10/CIFAR100/AID for self-training of ReCLIP, and then evaluate ReCLIP on the corresponding test sets from Table \ref{tab:main}. Results from Table \ref{generalization} indicates ReCLIP maintains its classification accuracy on the unseen examples. Therefore, ReCLIP is capable of accommodating new examples from the target domain without re-training.

    % \begin{table}[ht]
    % \setlength{\tabcolsep}{0.2em}
    % \centering
    % %\resizebox{\linewidth}{!}{
    % \begin{tabular}{cccc}
    %                       & CIFAR10 & CIFAR100 & AID   \\ \hline
    % CLIP                  & 95.60   & 78.22    & 68.73 \\
    % ReCLIP (Transductive) & 97.04   & 83.42    & 79.27 \\
    % ReCLIP (Inductive)    & 96.92   & 82.30    & 79.87 \\ \hline
    % \end{tabular}
    % %}
    % \caption{Effectiveness of ReCLIP in unseen sample (inductive setting). }
    % \label{generalization}
    % \end{table}


    % \subsubsection{Comparison of Learnable Modules}
    % In Table \ref{modules}, we evaluate different learnable modules by comparing their fully-supervised fine-tuned performance. As suggested in \cite{wang2020tent}, fine-tuning the normalization weights is shown to be efficient and stable, compared to fine-tuning the entire weights in self-training of ReCLIP. 
    % Recent research \cite{jia2022visual} also suggests that learnable prompts can also be effective in providing stable and fast performance improvement during the fine-tuning of Transformer \cite{vaswani2017attention, dosovitskiy2020image} based models. In Table \ref{modules}, we perform Visual Prompt tuning following \cite{jia2022visual}, and our own designed Text Prompt. Due to the space capacity, details of the learnable text prompt will be covered in the supplementary material. 
    
    % As shown in Table \ref{modules}, fine-tuning Layer-Norm weights from Visual Encoder has the best fully supervised accuracy on both CIFAR10 and CIFAR100, while fine-tuning Layer-Norm weights from Text Encoder has the best fully supervised accuracy on AID. As described in Section \ref{limitation_clip}, on some datasets (including AID), the performance CLIP is mainly limited by the poor quality text embeddings from inaccurate class names. In this case, fine-tuning the text encoder will achieve better performance as we observed. Table \ref{modules} results suggest the necessity of fine-tuning CLIP from both the visual and text side to handle different scenarios. 

    % \begin{table}[t]
    % \resizebox{\linewidth}{!}{
    %     \begin{tabular}{ccccc}
    %                                                         & CIFAR10       & CIFAR100          & AID        & SUN397   \\ \hline
    %     Vanilla CLIP                                        & 95.54         & 76.48             & 64.87      & 67.25   \\
    %     Learnable Text Prompts                              & 97.50          & 82.18            & 93.73      & 75.27   \\
    %     Learnable Visual Prompts \cite{jia2022visual}       & 96.70          & 80.68            & 74.27      & 68.09   \\
    %     Text Encoder Layer-Norm                             & 97.32         & 83.30             & \textbf{94.8} & \textbf{78.47} \\
    %     Visual Encoder Layer-Norm                           & \textbf{97.8} & \textbf{85.16}    & 69.40        & 68.30 \\ \hline  
    %     \end{tabular}
    % }
    % \caption{Fully supervised fine-tuning accuracy of CLIP with different learnable modules on ablation datasets. On AID, fine-tuning weights from Text Encoder Layer-Norm is shown to be most effective; On CIFAR10 and CIFAR100, fine-tuning weights from Visual Encoder Layer-Norm is shown to be most effective.}
    % \label{modules}
    % \end{table}
